CachePerf: A Unified Cache Miss Classifier via Hybrid Hardware Sampling

The cache plays a key role in determining the performance of applications, no matter for sequential or concurrent programs on homogeneous and heterogeneous architecture. Fixing cache misses requires to understand the origin and the type of cache misses. However, this remains to be an unresolved issue even after decades of research. This paper proposes a unified profiling tool--CachePerf--that could correctly identify different types of cache misses, differentiate allocator-induced issues from those of applications, and exclude minor issues without much performance impact. The core idea behind CachePerf is a hybrid sampling scheme: it employs the PMU-based coarse-grained sampling to select very few susceptible instructions (with frequent cache misses) and then employs the breakpoint-based fine-grained sampling to collect the memory access pattern of these instructions. Based on our evaluation, CachePerf only imposes 14% performance overhead and 19% memory overhead (for applications with large footprints), while identifying the types of cache misses correctly. CachePerf detected 9 previous-unknown bugs. Fixing the reported bugs achieves from 3% to 3788% performance speedup. CachePerf will be an indispensable complementary to existing profilers due to its effectiveness and low overhead.

==> relatedwork-capacitymiss_old_.tex <==


Dyer et al. proposes a strategy to reduce capacity misses by changing the placement and insertion policies of the cache~\cite{setSaturationLevels}. However, their strategy is fully based on the concept of the Set Saturation Level (SSL), which is provided by dynamic set balance cache (DSBC) only~\cite{setBalancingCache}. Thus, it is not a general method to profile and improve applications.

Tao et al. proposes a cache simulator, which can identify cache capacity misses using the reuse distance for each memory access~\cite{cacheSimulation}. And then proposed a toolset that covers the whole feedback loop of code optimization based on this tool.\cite{datalocalitytoolkit} However, the cache simulator can not be used as an online profiler, since its detection of cache capacity misses requires data of every memory access, which can introduce unacceptable performance overhead. Nikos et al. proposes another cache simulation methodology. Delorean~\cite{delorean} detects cache capacity misses by stack distance, which is the number of distinct memory accesses since the last access to the observed cacheline. However, it also requires inspection of every memory access. Both cache simulators are designed for studying cache behaviors under various cache configurations, and neither of them can be used as a profiling tool to improve applications.

Sanchez et al. proposes a data locality analysis tool, which can identify compulsory, conflict and capacity misses.\cite{SPLAT} However, a specialized compiler must be used to extract reuse information. The profiling stage incurs 10\% overhead, and the profiling results require offline processing. These characteristics make this tool inconvenient and inefficient to use.

Tao et al. proposes a cache simulator, which can identify cache capacity misses using the reuse distance for each memory access~\cite{cacheSimulation}. However, the cache simulator can not be used as an online profiler, since its detection of cache capacity misses requires data of every memory access, which can introduce unacceptable performance overhead. Nikos et al. proposes another cache simulation methodology Delorean~\cite{delorean}. The method detects cache capacity misses by stack distance, which is the number of distinct memory accesses since the last access to the observed cacheline. However, it also requires inspection of every memory access. Both the two cache simulations are designed for studying cache behaviors under various cache configurations, and neither of them can be used as a profiling tool to improve applications.

Dyer et al. proposes a strategy to reduce capacity misses by changing the placement and insertion policies of the cache~\cite{setSaturationLevels}. However, their strategy is fully based on the concept of the Set Saturation Level (SSL), which is provided by dynamic set balance cache (DSBC) only~\cite{setBalancingCache}. Thus, the it is not a general method to profile and improve applications.

